Principles of Quantum Universe

The present monograph is devoted to the theory of gravitation derived consequently as joint nonlinear realization of conformal and affine symmetries by means of Cartan differential forms. In the framework of the joint nonlinear realization of conformal and affine symmetries the interpretation of the last cosmological observational data of Ia Supernovae, anisotropy of the primordial radiation temperature and the mass spectrum of electroweak bosons, including the Higgs particle mass in the expected region ~ 125 GeV, is given. All these observational and experimental data testify to the vacuum energy dominance. The vacuum Casimir energy is a source of intensive cosmological quantum creation gravitons and electroweak bosons including Higgs particles from the empty Universe during the first 10^(-12) sec. The products of decay of the electroweak bosons give the matter content of the present day Universe, including primordial radiation and its baryon asymmetry.

==> QU17-ENG.tex <==
\makeatletter
\renewcommand{\@evenhead}{}
\renewcommand{\@oddhead}{}
\makeatother

\newpage

\newpage
\centerline{\bf PRINCIPLES OF QUANTUM~UNIVERSE}

%\vspace{1cm}

\begin{center}
{V.N. Pervushin,  A.E. Pavlov\\
Bogoliubov Laboratory of Theoretical Physics,\\
Joint Institute for Nuclear Research, 141980 Dubna, Russia}
\end{center}

%\vspace{1cm}
%
%\begin{flushright}
%\textit{
%1. In the beginning God created the heavens and the earth.\\
%2. The earth was without form, and void; \\ and darkness was on the face of the deep.\\
%And the Spirit of God was hovering over the face of the waters.\\
%3. Then God said:\\ ``Let there be light''; \\ and there was light.\\
%4. And God saw the light, that it was good;\\
%and God divided the light from the darkness.\\
%5. God called the light Day,  \\ and the darkness He called Night.\\
%So the evening and the morning were \\ the first day.\\
%} \vskip .5cm THE FIRST BOOK OF MOSES CALLED {\bf GENESIS}.
%\end{flushright}
%\vskip 2cm
%\begin

\centerline{ABSTRACT}

\vspace{.31cm}

{One of the main results of 20th century in astrophysics and cosmology was the revelation
of observational data testifying to the \textit{Beginning} of the Universe. In the end of 20th century
and beginning of the present one there were appeared that the Universe
was {void} (empty) in the Beginning. The Universe together with its matter was arisen from
\textit{nothing}. In the modern theories, this genesis from \textit{nothing} can be described
by means of quantization of the gravitation field with a postulate of existence of \textit{vacuum}
as a state of energy minimum. Hence, the theory of gravitation adequate describing the Universe being arisen
from the vacuum is to be quantum. A possibility of construction of quantum theory of gravitation is
appeared if it is being derived consequently from ab initio:
joint affine and conformal groups of symmetry laid in the base of the initial classical theory.
The monograph is devoted to classical and quantum theories of gravitation which are derived by joint
nonlinear realization of conformal and affine symmetries by Cartan linear forms.
In terms of Cartan forms the actions of the theory of gravitation and the Standard Model of
electroweak interactions describe a system of squeezed oscillators with nonconserved numbers of
occupations. This system of squeezed oscillators admits quantization of all fields including
the gravitation and and the scalar Higgs field on an equal footing. The Casimir energy is a source
of intensive cosmological quantum creation of $\sim 10^{90}$ gravitions and Higgs particles from
vacuum of empty Universe during $10^{-12}$ sec. Products of their decay give the matter content
of the present day Universe including primordial radiation.
The uncertainty principle of action at the Planck's epoch within our model defines the
red shift value at the moment of birth of our Universe and sets the hierarchy of the Universe energy scales,
including the Hubble parameter, primordial radiation temperature, mass scales of the Standard Model and
the Plank's mass in according with the observational data. The interpretation of the last cosmological
observational data on Ia Supernovae, anisotropy of the primordial radiation temperature and the mass
spectrum of electroweak bosons including the Higgs particle mass in the expected region 130$\pm 15$ GeV
is given in frame of our approach.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%}
%
%{\small
%One of the main results of research in astrophysics and cosmology in the 20th century was the revelation
%of observational data testifying to the \textit{Beginning} of the Universe. It is generally accepted that
%at the end of the 20th century and at the beginning of the present one there appeared new facts proclaiming that
%the Universe was void at the Beginning. The Universe together with its matter arose from
%\textit{nothing}. This genesis from \textit{nothing} (id est from the \textit{vacuum} in modern physics language)
%can be described by means of quantization of the gravitation field. Hence, the theory of gravitation
%adequately describing the Universe genesis is to be {\it quantum} with a postulate of the existence of the
%\textit{vacuum} as a state of energy minimum. A possibility of construction of the
%{\it quantum} theory of gravitation appears if the initial classical theory of gravitation is to be derived
%consequently as joint nonlinear realization of conformal and affine symmetries by means of Cartan differential
%forms and then to be quantized in terms of these forms. In the framework of the joint
%nonlinear realization of conformal and affine symmetries the interpretation of the last cosmological
%observational data of Ia Supernovae, anisotropy of the primordial radiation temperature and the mass
%spectrum of electroweak bosons, including the Higgs particle mass in the expected region 130$\pm 15$ GeV,
%is given. All these observational and experimental data testify to the vacuum energy dominance.
%Under the condition of dominance of the vacuum Casimir energy in the empty space
%the Planck principle of minimal action defines the red shift value
%$z_{I}\sim 10^{15}$ and its velocity at the  initial moment of the Universe's birth.
%The initial data of the red shift and its velocity set the hierarchy of the energy scales,
%including the Hubble parameter, primordial radiation temperature,
%mass scales of the Standard Model of elementary particles and the Plank mass, in accordance with the
%observational data.
%In the joint nonlinear realization of conformal and affine symmetries the actions of the theory of gravitation
%and the Standard Model of the electroweak interactions describe a system of squeezed oscillators
%with non-conserved numbers of occupations of gravitons and Higgs particles. The vacuum Casimir energy is a
%source of intensive cosmological quantum creation of $\sim 10^{90}$ gravitons and electroweak bosons including
%Higgs particles from the empty Universe during the first $10^{-12}$ sec. The products of decay of the
%electroweak bosons
%give the matter content of the present day Universe, including primordial radiation and its baryon asymmetry.
%
%}

\centerline{АННОТАЦИЯ}
\vspace{1cm}

{\small Одним из самых главных результатов исследований в астрофизике и космологии  XX
века было открытие наблюдательных данных, свидетельствующих о \textit{начале} Вселенной.
Общепринято считать, что в конце XX века и начале нынешнего появились новые факты, говорящие о том, что
в начале Вселенная была \textit{пустой}. Вселенная вместе с её материей возникла из
\textit{ничего}. Возникновение из \textit{ничего} (то есть из \textit{вакуума} на языке
современной физики) может быть описано посредством квантования гравитационного поля.
Следовательно, теория гравитации, адекватно описывающая возникновение Вселенной, должна быть
\textit{квантовой} с постулатом существования \textit{вакуума} как состояния с наименьшей
энергией. Как будет показано в настоящей монографии, возможность построения такой
\textit{квантовой} теории гравитации неизбежно возникает, если классическую теорию гравитации
последовательно вывести как  совместную нелинейную реализацию конформной и аффинной симметрий
посредством дифференциальных форм Картана, и затем квантовать в терминах этих форм.
В рамках этой совместной нелинейной реализации
 конформной и аффинной симметрий даётся интерпретация последних космологических наблюдательных
 данных по Сверхновым, анизотропии температуры реликтового излучения, а также  спектра масс
 электрослабых бозонов, включая частицы Хиггса с массой в интервале 130$\pm 15$ ГэВ.
Все эти наблюдательные и экспериментальные факты свидетельствуют о доминантности
 вакуумной энергии. При условии доминантности вакуумной энергии Казимира в
пустом пространстве
принцип минимального действия Планка определяет значение красного смещения $z_{I}\sim 10^{15}$ и его
скорость в начальный момент рождения Вселенной.  Начальные значения красного смещения и его скорости
 задают иерархию
энергетических масштабов, включая современные значения параметра Хаббла, температуры реликтового
излучения, масштаба  масс Стандартной Модели элементарных частиц и значение планковской массы в
соответствии с наблюдательными данными.
 В совместной нелинейной реализации конформной и аффинной симметрий действия гравитации и
 Стандартной Модели электрослабого взаимодействия описывают систему сжатых осцилляторов с
 несохраняющимися числами заполнения гравитонов и частиц Хиггса. Вакуумная энергия Казимира
 является источником интенсивного космологического квантового рождения $\sim 10^{88}$ гравитонов
 и электрослабых бозонов, в том числе и частиц Хиггса, в пустой Вселенной в течении $10^{-12}$
 сек. Распады электрослабых бозонов дают  материальное содержание современной Вселенной, включая
 реликтовое излучение и её барионную асимметрию.}

%В настоящей монографии показано, что возможность построения \textit{квантовой} теории
%гравитации неизбежно возникает, если классическую теорию гравитации последовательно вывести как
%совместную нелинейную реализацию конформной и аффинной симметрий посредством дифференциальных форм Картана,
%и затем квантовать в терминах этих форм. В рамках такой \textit{квантовой} теории Вселенной строится оператор
% рождения и эволюции Вселенной и дана классификация состояний полей материи, которая включает светимость
% космических объектов как параметр эволюции в полевом пространстве событий. Средние от оператора рождения
% и эволюции Вселенной описывают процессы рождения материи из вакуума в согласии с современными космологическими
%  наблюдательными
% данными, включая данные по Сверхновым,  и
%дают соответствие между параметрами космологии и физики элементарных частиц, включая значение массы
%частицы Хиггса  в интервале 130$\pm 15$ ГэВ
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\begin{center}
{\bf \large\bf Victor Nikolaevich Pervushin}
\end{center}

 the Directorate Councillor of the Bogoliubov Laboratory of Theoretical Physics, Joint Institute for
 Nuclear Researches,
Professor, is known by his papers devoted to:\\
$\blacklozenge$ the foundation of eikonal scattering amplitude in quantum field theory,
 recognized by the most prestige USSR Prize for young scientists together with Academicians
 V.A. Matveev and A.N. Sisakian (1973);\\
 $\blacklozenge$ the formulation of the chiral perturbation theory for
 low-energy physics of mesons expounded together with Prof. M.K.Volkov in the monograph
 `\textit{Essentially Nonlinear Field Theory, Dynamical Symmetry and Meson Physics}`
 published under the editorship of the prominent Soviet physicist D.I. Blokhintsev (1978);\\
 $\blacklozenge$ the proposal of the successful measurement of the pion polarizability at
 the Serpukhov Accelerator marked by
 the First Award of JINR for scientific achievements in  1987;\\
 $\blacklozenge$  the collective variables
  describing the spontaneous chiral symmetry breaking in QCD and
   bilocal mesons in hot and dense medium (the Max Planck Society Grand of 1989--2000));  \\
 %the development of the Dirac quantization of gauge theories based on their
% Poincar\'e classification with  topological degeneration of initial data (the Max Planck Society Grand).\\
%  the description of bilocal mesons in hot and dense medium (the Max Planck Society Grand). \\
  $\blacklozenge$ the description of the Supernova data on the redshift -- luminosity-distance relation
   within the Conformal Cosmology without Inflation and Lambda term (cited by A. Riess in his
   2010-Nobel Prise  paper of 2001);
    \\
   $\blacklozenge$  the effect of intensive cosmological creation of the
    SM bosons (catalyzing the baryon asymmetry) as the origin of the present
    matter content of the Universe (the Max Planck Society Grand of 2001);\\
     %2002 - 2008: The discovery of the effect of capture of cosmic objects by central
%     field due to cosmic evolution and the large - scale structure of the Universe.\\
%      2006 - 2012: The formulation (with coauthors) of the Conformal and Affine General Relativity
%      for  the Early Universe evolution.\\
$\blacklozenge$ the prediction of the kaon decay branching into pion and lepton pair, confirmed
in NA-48 measurement  at
the CERN Accelerator (the Second Award of JINR for scientific achievements in 2011).
%Recent awards include the International Plato Award for Educational Achievement (2011). %,\\
%and nomination as International Biographical Center Man of the Year (2011), Cambridge, England.
\vskip 1cm
\begin{center}
{\bf\large\bf Alexander Egorovich Pavlov}
\end{center}

--  associated professor of the department of theoretical mechanics of Moscow Agri -- Engineering University,
PhD, theoretical physicist, author of 50 scientific papers? published in ``Physics Letters'', ``International
Journal of Modern Physics'', ``International Journal of Theoretical Physics'', etc. His interests: quantum
gravitation, quantum field theory, theoretical mechanics, etc. Author of textbooks and monographs (in Russian):
\textit{Hamiltonian Dynamics of Point Vortices},
\textit{Conspectus of lectures on theoretical mechanics},
\textit{Dynamics of rigid body of elliptic form},
\textit{Selected problems of theoretical mechanics},
\textit{Elements of mathematical statistics}.

\newpage

%\medskip
%\end{center}
%\subsubsection*{\bf ACADEMIC DEGREES}
% \begin{enumerate}
%\item[]
%       \begin{tabbing}
%          1978 \,\, \= D.\,Sc.,
%           %\hnl{Laboratory of Theoretical Physics}{http://bltp.jinr.ru/},
%                   Dubna, Russia\\
%               \>  Title: %\hnl
%               {``Quantum Field Theory for Chiral Lagrangian
%               and Low-- Energy Meson Physics''}
%               %{http://www.dissercat.com/content/QFT~for~low~energy~meson~physics}
%                    \end{tabbing}
%  \item[]
%       \begin{tabbing}
%          1970 \,\, \= Ph.\,D.,
%           %\hnl
%           {Laboratory of Theoretical Physics}{http://www.pfu.edu.ru/},
%                   Moscow, Russia\\
%               \>  Title: %\hnl
%               {``Foundation of Eikonal
%    Approximation in Quantum Field Theory''
%}%{http://www.dissercat.com/content/eikonal~
%%    approximation~ in~ quantum~ field~ theory}
%\\
%               \>    Supervisor: Profs. D.I. Blokhintsev
%    and B.M. Barbashov.
%      \end{tabbing}
 %\item[]
%       \begin{tabbing}
%          1989 \,\, \= M.\,Sc.,
%           \hnl{Russian Peoples' Friendship University}{http://www.pfu.edu.ru/},
%                   Moscow, Russia\\
%               \>  Title: "Interaction of charged solitons with
%Coulomb center" \\
%               \>    Supervisor: Prof. Yu. P. Rybakov.
%      \end{tabbing}


%  \end{enumerate}

%
%\subsubsection*{\bf FIELDS OF SPECIALIZATION}
%  \begin{enumerate}
%  \item[] QFT, GR, cosmology of Early Universe, QCD at low energy region
%
%  \end{enumerate}

%\subsubsection*{\bf EDUCATION}
% Ba in Physics, Lomonosov State University, Moscow, Russia, 1968\\
%PhD in Physics and Mathematics, Joint Institute for Nuclear Researches, 1970\\
%ScD in Physics and Mathematics, Joint Institute for Nuclear Researches, 1978

%
%\subsubsection*{\bf PROFESSIONAL CAREER:}
%
%1971 - 1975: Staff member of Joint Institute for Nuclear Research (JINR).\\
%1975 - 1989: Senior researcher, JINR.\\
%1989 - 2007: Head of Sector N 5, Bogoliubov Laboratory of Theoretical Physics, JINR.\\
%Professor of Theoretical Physics since 1989.\\
%2008 - Present: the Directorate Councillor of the Bogoliubov Laboratory of Theoretical Physics, JINR.
%{http://theor.jinr.ru/~pervush}
%
%\section*
%\begin{center}
%\begin{figure}[ht]
%\centerline{\includegraphics[width=0.45\textwidth]{Pervushin2.eps}}
%\end{figure}
%\end{center}


%\begin{figure}[htb!]
%\begin{center}
%\includegraphics[width=0.5\textwidth]{Pervushin2.eps}
%\end{center}
%%\caption
%{\footnotesize Виктор  Николаевич Первушин
%— профессор, доктор физико--математических наук,
%консультант Дирекции Лаборатории теоретической физики им. Н.Н. Боголюбова Объединённого
%института ядерных исследований, известен своими работами по\\
%$\blacklozenge$ обоснованию эйкональной амплитуды рассеяния в квантовой теории поля,
%за которое присуждена  Премия Ленинского Комсомола в 1973 г.
%совместно с академиками В.А. Матвеевым и А.Н. Сисакяном;\\
%$\blacklozenge$ формулировке широко используемой киральной теории возмущения,
%изложенной  с проф. М.К. Волковым в монографии
%\textit{Существенно нелинейные теории поля, динамические симметрии и физика мезонов},
%опубликованной под редакцией
%Д.И. Блохинцева в 1978 г.;\\
%$\blacklozenge$ успешному измерению поляризуемости пионов на Серпуховском ускорителе,
%отмеченному с группой авторов
%первой премией ОИЯИ в 1987 г.;\\
%$\blacklozenge$
%билокальному описанию мезонов в горячей и плотной среде
%(the Max Planck Society Grand of 1989--2000);\\
%$\blacklozenge$  описанию данных по Сверхновым в Конформной космологии без инфляции и лямбда-члена,
%цитированному Нобелевским лауреатом  А. Риссом (2010 г.) в его работе 2001 г.;\\
%$\blacklozenge$ эффекту интенсивного космологического рождения
%электрослабых бозонов с  барионной асимметрией (the Max Planck Society Grand of 2001);\\
%$\blacklozenge$ исследованию  электрослабых распадов каонов, вероятности которых в борновском приближении
%равны нулю,
%на ускорителе в ЦЕРНе (NA/48), отмеченному с группой соавторов
%второй премией ОИЯИ в 2011 г.
%}
%\end{figure}

%\newpage
\begin{center}
{\vspace{0.31cm}}
\parbox{0.5\textwidth}{
\includegraphics[height=8.truecm,
angle=-0]{Pervushin2.eps}}
\parbox{0.48\textwidth}
{\footnotesize
Виктор  Николаевич Первушин
— профессор, доктор физико--математических наук,
консультант Дирекции Лаборатории теоретической физики им. Н.Н. Боголюбова Объединённого
института ядерных исследований, известен своими работами по\\
$\blacklozenge$ обоснованию эйкональной амплитуды рассеяния в квантовой теории поля,
%за которое присуждена  Премия Ленинского Комсомола в 1973 г.
совместно с академиками В.А. Матвеевым и А.Н. Сисакяном;\\
$\blacklozenge$ формулировке широко используемой
квантовой киральной теории возмущения, %для низко-энергетической физики мезонов,
изложенной  с проф. М.К. Волковым в монографии
\textit{Существенно нелинейные теории поля, динамические симметрии и физика мезонов},
опубликованной под редакцией
Д.И. Блохинцева в 1978 г.;\\
%$\blacklozenge$ успешному измерению поляризуемости пионов на Серпуховском ускорителе,
%отмеченному с группой авторов
%первой премией ОИЯИ в 1987 г.;\\
%$\blacklozenge$
%  билокальному описанию мезонов в горячей и плотной среде (the Max Planck Society Grand of 1989--2000);
%  \\
$\blacklozenge$  описанию данных по Сверхновым в Конформной космологии без инфляции и лямбда-члена
(цитированному Нобелевским лауреатом  А. Риссом (2010 г.) в его работе 2001 г.
%$\blacklozenge$ эффекту интенсивного космологического рождения
%электрослабых бозонов с  барионной асимметрией (the Max Planck Society Grand of 2001).
%$\blacklozenge$ исследованию  электрослабых распадов каонов, вероятности которых в борновском приближении
%равны нулю,
%на ускорителе в ЦЕРНе (NA/48), отмеченному с группой соавторов
%второй премией ОИЯИ в 2011 г.
}
{\vspace{0.31cm}}
\end{center}


\begin{center}
%{\vspace{0.31cm}}
\parbox{0.5\textwidth}{
\includegraphics[height=5truecm,
angle=-0]{Pavlov2.eps}}
\parbox{0.48\textwidth}
{\footnotesize Павлов Александр Егорович --
доцент кафедры теоретической механики им. Н.И. Мерцалова МГАУ, кандидат физико--математических наук.
Физик--теоретик, автор более 50 научных работ, опубликованных в ``Physics Letters'', ``International
Journal of Modern Physics'', ``International Journal of Theoretical Physics'' и др.
В круг его научных интересов входят квантовая гравитация,
квантовая теория поля, теоретическая механика. Автор
учебников и монографий по теоретической механике:
\textit{Гамильтонова динамика точечных вихрей},
\textit{Конспект лекций по теоретической механике},
\textit{Динамика твёрдого тела эллипсоидной формы},
\textit{Избранные задачи теоретической механики},
\textit{Элементы математической статистики}.
}
\end{center}
%\vspace{2cm}
%{\bf \large\bf Павлов Александр Егорович}

%\begin{center}
%\begin{figure}[ht]
%\includegraphics[width=0.5\textwidth]{Pavlov2.eps}
%%\caption
%{\footnotesize Павлов Александр Егорович --
%доцент кафедры теоретической механики им. Н.И. Мерцалова МГАУ, кандидат физико--математических наук.
%Физик--теоретик, автор более 50 научных работ, опубликованных в ``Physics Letters'', ``International
%Journal of Modern Physics'', ``International Journal of Theoretical Physics'' и др.
%В круг его научных интересов входят квантовая гравитация,
%квантовая теория поля, теоретическая механика. Автор
%учебников и монографий по теоретической механике:
%\textit{Гамильтонова динамика точечных вихрей},
%\textit{Конспект лекций по теоретической механике},
%\textit{Динамика твёрдого тела эллипсоидной формы},
%\textit{Избранные задачи теоретической механики},
%\textit{Элементы математической статистики}.
%}
%\end{figure}
%\end{center}

%\begin{figure}[htb!]
%\begin{center}
%\includegraphics[width=.6\textwidth]{Pavlov2.eps}
%\end{center}
%%\caption
%{\footnotesize Павлов Александр Егорович --
%доцент кафедры теоретической механики им. Н.И. Мерцалова МГАУ, кандидат физико--математических наук.
%Физик--теоретик, автор более 50 научных работ, опубликованных в ``Physics Letters'', ``International
%Journal of Modern Physics'', ``International Journal of Theoretical Physics'' и др.
%В круг его научных интересов входят квантовая гравитация,
%квантовая теория поля, теоретическая механика. Автор
%учебников и монографий по теоретической механике:
%\textit{Гамильтонова динамика точечных вихрей},
%\textit{Конспект лекций по теоретической механике},
%\textit{Динамика твёрдого тела эллипсоидной формы},
%\textit{Избранные задачи теоретической механики},
%\textit{Элементы математической статистики}.
%}
%\end{figure}
%\begin{center}
%{\vspace{0.31cm}}
%\parbox{0.58\textwidth}{
%\includegraphics[height=7.truecm,
%angle=-0]{Pavlov2.eps}}
%\parbox{0.38\textwidth}
%{\small Павлов Александр Егорович --
%доцент кафедры теоретической механики им. Н.И. Мерцалова МГАУ, кандидат физико--математических наук.
%Физик--теоретик, автор более 50 научных работ, опубликованных в ``Physics Letters'', ``International
%Journal of Modern Physics'', ``International Journal of Theoretical Physics'' и др.
%В круг его научных интересов входят квантовая гравитация,
%квантовая теория поля, теоретическая механика. Автор
%учебников и монографий по теоретической механике:
%\textit{Гамильтонова динамика точечных вихрей},
%\textit{Конспект лекций по теоретической механике},
%\textit{Динамика твёрдого тела эллипсоидной формы},
%\textit{Избранные задачи теоретической механики},
%\textit{Элементы математической статистики}.

%Виктор  Николаевич Первушин
%— профессор, консультант Дирекции Лаборатории теоретической физики им. Н.Н. Боголюбова Объединённого
%института ядерных исследований, известен своими работами по\\
%$\blacklozenge$ обоснованию эйкональной амплитуды рассеяния в квантовой теории поля,
%за которое присуждена  Премия Ленинского Комсомола в 1973 г.
%совместно с академиками В.А. Матвеевым и А.Н. Сисакяном;\\
%$\blacklozenge$ формулировке широко используемой киральной теории возмущения, %для низко-энергетической физики мезонов,
%изложенной  с проф. М.К. Волковым в монографии
%\textit{Существенно нелинейные теории поля, динамические симметрии и физика мезонов},
%опубликованной под редакцией
%Д.И. Блохинцева в 1978 г.;\\
%$\blacklozenge$ успешному измерению поляризуемости пионов на Серпуховском ускорителе,
%отмеченному с группой авторов
%первой премией ОИЯИ в 1987 г.;\\
%$\blacklozenge$
%  билокальному описанию мезонов в горячей и плотной среде (the Max Planck Society Grand of 1989--2000);
%  \\
%$\blacklozenge$  описанию данных по Сверхновым в Конформной космологии без инфляции и лямбда-члена
%(цитированному Нобелевским лауреатом  А. Риссом (2010 г.) в его работе 2001 г.;\\
%$\blacklozenge$ эффекту интенсивного космологического рождения
%электрослабых бозонов с  барионной асимметрией (the Max Planck Society Grand of 2001);\\
%$\blacklozenge$ исследованию  электрослабых распадов каонов, вероятности которых в борновском приближении
%равны нулю,
%на ускорителе в ЦЕРНе (NA/48), отмеченному с группой соавторов
%второй премией ОИЯИ в 2011 г.
%}
%{\vspace{0.31cm}}
%\end{center}
%\begin{center}
%\begin{figure}[ht]
%\includegraphics[width=0.6\textwidth]{Pavlov2.eps}
%\end{figure}
%\end{center}

